Ensuring Visual Commonsense Morality for Text-to-Image Generation

Text-to-image generation methods produce high-resolution and high-quality images, but these methods should not produce immoral images that may contain inappropriate content from the perspective of commonsense morality. In this paper, we aim to automatically judge the immorality of synthesized images and manipulate these images into morally acceptable alternatives. To this end, we build a model that has three main primitives: (1) recognition of the visual commonsense immorality in a given image, (2) localization or highlighting of immoral visual (and textual) attributes that contribute to the immorality of the image, and (3) manipulation of an immoral image to create a morally-qualifying alternative. We conduct experiments and human studies using the state-of-the-art Stable Diffusion text-to-image generation model, demonstrating the effectiveness of our ethical image manipulation approach.

==> src/related_work.tex <==
\vspace{-.5em}
There has been a long effort to build the concept of ethical machine learning~\cite{asimov1941three, bostrom2012superintelligent, awad2018moral}. Recently, AI ethics have become a more apparent interest of importance in AI and CV communities. From Natural Language Processing (NLP) community, an increasing number of papers have been introduced, examining five different ethical categories: (i) Fairness~\cite{kleinberg2016inherent}, (ii) Safety~\cite{ray2019benchmarking}, (iii) Prosocial~\cite{roller2020recipes}, (iv) Utility~\cite{christiano2017deep}, and (v) Commonsense Morality~\cite{hendrycks2020aligning}. Especially the last topic, commonsense morality, has limited been explored in the computer vision community, which mainly focuses on safety~\cite{wu2020not} and fairness ~\cite{park2022fair, sirotkin2022study}. Thus, this paper focuses on commonsense morality from the computer vision perspective. Our work starts by analyzing state-of-the-art text-to-image generation model, Stable Diffusion, and we propose a novel ethical image manipulation approach to edit the {\em immorally} generated image into a {\em moral} one. We provide a more detailed explanation of text-driven image generation models and their social impact in Appendix~\ref{sec:appendix-related_works}.


